BB: Booting Booster for Consumer Electronics with Modern OS

Unconventional computing platforms have spread widely and rapidly following smart phones and tablets: consumer electronics such as smart TVs and digital cameras. For such devices, fast booting is a critical requirement; waiting tens of seconds for a TV or a camera to boot up is not acceptable, unlike a PC or smart phone. Moreover, the software platforms of these devices have become as rich as conventional computing devices to provide comparable services. As a result, the booting procedure to start every required OS service, hardware component, and application, the quantity of which is ever increasing, may take unbearable time for most consumers. To accelerate booting, this paper introduces \textit{Booting Booster} (BB), which is used in all 2015 Samsung Smart TV models, and which runs the Linux-based Tizen OS. BB addresses the init scheme of Linux, which launches initial user-space OS services and applications and manages the life cycles of all user processes, by identifying and isolating booting-critical tasks, deferring non-critical tasks, and enabling execution of more tasks in parallel. BB has been successfully deployed in Samsung Smart TV 2015 models achieving a cold boot in 3.5 s (compared to 8.1 s with full commercial-grade optimizations without BB) without the need for suspend-to-RAM or hibernation. After this successful deployment, we have released the source code via http://opensource.samsung.com, and BB will be included in the open-source OS, Tizen (http://tizen.org).

==> old/disabled-generated.bbl.tex <==
\begin{thebibliography}{}
\softraggedright

\bibitem[Son()]{Sony_Android_TV}
Bravia with android tv™.
\newblock \url{https://developer.sony.com/develop/tvs/android-tv/}.
\newblock Accessed: 2015-10-21.

\bibitem[boo({\natexlab{a}})]{boot_time_hisense_40s}
Review: Hisense 55” android-powered smart tv.
\newblock
  \url{http://techau.com.au/review-hisense-55-android-powered-smart-tv/comment-page-1/},
  {\natexlab{a}}.
\newblock Accessed: 2015-10-21.

\bibitem[boo({\natexlab{b}})]{boot_time_sonytv_20s}
Sony community (televisions).
\newblock
  \url{https://community.sony.nl/t5/televisions/w800b-software-is-so-slow-you-have-to-wait-15-seconds-before-hdmi/td-p/1661837},
  {\natexlab{b}}.
\newblock Accessed: 2015-10-21.

\bibitem[bui()]{build-external-module}
Building external modules.
\newblock \url{https://www.kernel.org/doc/Documentation/kbuild/modules.txt}.
\newblock Accessed: 2016-2-8.

\bibitem[bus()]{busybox-init}
Busybox.
\newblock \url{http://sourceforge.net/projects/einit/}.
\newblock Accessed: 2015-09-30.

\bibitem[cod()]{codeviz}
A callgraph visualiser.
\newblock \url{http://ww.csn.ul.ie/~mel/projects/codeviz}.
\newblock Accessed: 2015-10-01.

\bibitem[cre()]{creating-rcs-script}
Creating the rcs script.
\newblock
  \url{http://archive.linuxfromscratch.org/lfs-museum/3.1/LFS-BOOK-3.1-HTML/chapter07/rcs.html}.
\newblock Accessed: 2016-2-8.

\bibitem[crt()]{crt}
Cathode ray tube: General description.
\newblock \url{http://www.newworldencyclopedia.org/entry/Cathode_ray_tube}.
\newblock Accessed: 2015-10-01.

\bibitem[dbu()]{dbus}
D-bus tutorial.
\newblock \url{http://dbus.freedesktop.org/doc/dbus-tutorial.html}.
\newblock Accessed: 2015-10-14.

\bibitem[deb({\natexlab{a}})]{debian_fork_devuan}
Devuan gnu/linux - debian without systemd.
\newblock \url{https://devuan.org}, {\natexlab{a}}.
\newblock Accessed: 2015-09-30.

\bibitem[deb({\natexlab{b}})]{debugging-by-printing}
Debugging by printing.
\newblock \url{http://elinux.org/Debugging_by_printing}, {\natexlab{b}}.
\newblock Accessed: 2015-10-14.

\bibitem[ein()]{einit}
einit.
\newblock \url{http://sourceforge.net/projects/einit/}.
\newblock Accessed: 2015-09-30.

\bibitem[emm()]{emmc_to_ufs}
emmc to ufs: How nand memory for mobile products is evolving.
\newblock
  \url{http://global.samsungtomorrow.com/emmc-to-ufs-how-nand-memory-for-mobile-products-is-evolving/}.
\newblock Accessed: 2015-10-01.

\bibitem[eve()]{everspin_mram_low_cost}
Magnetoresistive random access memory (mram) devices.
\newblock \url{http://www.digikey.com/catalog/en/partgroup/parallel-mram/1499}.
\newblock Accessed: 2015-10-15.

\bibitem[fas()]{fast_warmup_picture}
Fast warm up picture tube cathode cap having high heat emissivity surface on
  the interior thereof.
\newblock \url{https://www.google.com/patents/US3958146}.
\newblock Accessed: 2015-10-01.

\bibitem[gal({\natexlab{a}})]{galaxy_s6_geekbench}
Geekbench browser: Samsung sm-g925p.
\newblock \url{http://browser.primatelabs.com/geekbench3/1874253},
  {\natexlab{a}}.
\newblock Accessed: 2015-10-01.

\bibitem[gal({\natexlab{b}})]{galaxy_s6_ufs_benchmark}
{Samsung Galaxy S6} storage performance test.
\newblock
  \url{http://blog.gsmarena.com/samsung-galaxy-s6-storage-performance-test/},
  {\natexlab{b}}.
\newblock Accessed: 2015-10-01.

\bibitem[gra()]{graphviz}
Open source graph (network) visualization project from at\&t research.
\newblock \url{http://www.graphviz.org}.
\newblock Accessed: 2015-10-01.

\bibitem[idf()]{idf2015}
Intel developer forum 2015 (124 sessions).
\newblock
  \url{http://myeventagenda.com/sessions/0B9F4191-1C29-408A-8B61-65D7520025A8/7/5}.
\newblock Accessed: 2015-10-15.

\bibitem[inc()]{inconvenient_truth_of_nand}
The inconvenient truths about nand flash memory.
\newblock \url{http://arxiv.org/pdf/1208.6390.pdf}.
\newblock Accessed: 2015-10-01.

\bibitem[ini()]{init_definition}
Init.
\newblock \url{http://en.wikipedia.org/wiki/Init}.
\newblock Accessed: 2015-09-30.

\bibitem[ins({\natexlab{a}})]{instant_on_samsung_2s}
Samsung 55-inch hu7200 series 7 smart uhd led flat tv.
\newblock
  \url{http://www.samsung.com/uk/consumer/tv-audio-video/televisions/uhd-tvs/UE55HU7200UXXU},
  {\natexlab{a}}.
\newblock Accessed: 2015-10-21.

\bibitem[ins({\natexlab{b}})]{instant_warm_cathode}
Instant warm-up heater cathode.
\newblock \url{https://www.google.com/patents/US3895249}, {\natexlab{b}}.
\newblock Accessed: 2015-10-01.

\bibitem[lau()]{launchd}
einit.
\newblock \url{http://launchd.info/}.
\newblock Accessed: 2015-09-30.

\bibitem[lin()]{linux-start-scripts}
Linux startup scripts.
\newblock \url{https://luv.asn.au/overheads/linux-startup.html}.
\newblock Accessed: 2016-2-8.

\bibitem[mic()]{micron_3d_xpoint}
3d xpoint technology: Breakthrough nonvolatile memory technology.
\newblock \url{http://www.micron.com/about/innovations/3d-xpoint-technology}.
\newblock Accessed: 2015-10-14.

\bibitem[nx3()]{nx300_1.2sec_stratup}
Samsung nx300 performance.
\newblock
  \url{http://www.imaging-resource.com/PRODS/samsung-nx300/samsung-nx300A6.HTM}.
\newblock Accessed: 2015-10-13.

\bibitem[ope()]{opensource_samsung}
Samsung open source release center.
\newblock \url{http://opensource.samsung.com}.
\newblock Accessed: 2015-09-30.

\bibitem[pau()]{paul15_locking_performance}
Rcu vs. locking performance on different cpus.
\newblock \url{http://linux.conf.au}.
\newblock Accessed: 2015-09-30.

\bibitem[qui()]{quick_heating_cathode}
Quick-heating cathode structure.
\newblock \url{https://www.google.com/patents/US4388551}.
\newblock Accessed: 2015-10-01.

\bibitem[svs()]{svscan}
Svscan.
\newblock \url{http://cr.yp.to/daemontools/svscan.html}.
\newblock Accessed: 2015-09-30.

\bibitem[sys({\natexlab{a}})]{systemd_bootchart}
systemd-bootchart - boot performance graphing tool.
\newblock
  \url{http://www.freedesktop.org/software/systemd/man/systemd-bootchart.html},
  {\natexlab{a}}.
\newblock Accessed: 2015-10-20.

\bibitem[sys({\natexlab{b}})]{systemd_official_freedesktop}
systemd system and service manager.
\newblock \url{http://www.freedesktop.org/wiki/Software/systemd},
  {\natexlab{b}}.
\newblock Accessed: 2015-09-30.

\bibitem[sys({\natexlab{c}})]{systemd_unit}
systemd.unit - unit configuration.
\newblock
  \url{http://www.freedesktop.org/software/systemd/man/systemd-bootchart.html},
  {\natexlab{c}}.
\newblock Accessed: 2015-10-23.

\bibitem[sys({\natexlab{d}})]{systemd_wiki_adoption}
systemd, adoption and reception.
\newblock \url{http://en.wikipedia.org/wiki/Systemd#Adoption_and_reception},
  {\natexlab{d}}.
\newblock Accessed: 2015-09-30.

\bibitem[sys()]{sysvinit}
sysvinit.
\newblock \url{http://savannah.nongnu.org/projects/sysvinit}.
\newblock Accessed: 2015-09-30.

\bibitem[tiz()]{tizen_association}
Tizen project.
\newblock \url{http://www.tizen.org}.
\newblock Accessed: 2015-09-30.

\bibitem[tv_({\natexlab{a}})]{tv_market_share_2014}
Samsung, lg electronics took up 40% of global smart tv market last year.
\newblock
  \url{http://www.businesskorea.co.kr/features/focus/10104-smart-segment-domination-samsung-lg-electronics-took-40-global-smart-tv-market},
  {\natexlab{a}}.
\newblock Accessed: 2015-10-14.

\bibitem[tv_({\natexlab{b}})]{tv_market_share_2015Q1}
Samsung's share of global tv market edges down in q1.
\newblock
  \url{http://english.yonhapnews.co.kr/news/2015/05/19/0200000000AEN20150519003800320.html},
  {\natexlab{b}}.
\newblock Accessed: 2015-10-14.

\bibitem[tv_({\natexlab{c}})]{tv_market_share_2015Q2}
Samsung maintains top spot in global tv market.
\newblock
  \url{http://english.chosun.com/site/data/html_dir/2015/08/20/2015082001186.html},
  {\natexlab{c}}.
\newblock Accessed: 2015-10-14.

\bibitem[whe()]{where-nvram-fit}
Where does nvram fit?
\newblock \url{http://thessdguy.com/where-does-nvram-fit/}.
\newblock Accessed: 2015-10-15.

\bibitem[win()]{win-service-controller}
Windows service control manager: Automatically starting services.
\newblock
  \url{https://msdn.microsoft.com/en-us/library/windows/desktop/ms681957(v=vs.85).aspx}.
\newblock Accessed: 2016-2-8.

\bibitem[EU_(2013)]{EU_regulation_standby}
{Commission Regulation (EU) No 801/2013}.
\newblock
  \url{http://eur-lex.europa.eu/legal-content/EN/TXT/HTML/?uri=CELEX:32013R0801&from=EN},
  August 2013.
\newblock Accessed: 2015-10-23.

\bibitem[Adams et~al.(2005)Adams, Bustos, Hahn, Powell, and
  Praza]{adams05_solaris}
J.~Adams, D.~Bustos, S.~Hahn, D.~Powell, and L.~Praza.
\newblock Solaris service management facility: Modern system startup and
  administration.
\newblock In \emph{LISA}, pages 225--236, 2005.

\bibitem[Asberg et~al.(2013)Asberg, Nolte, Joki, Hogbrink, and
  Siwani]{asberg13_fast}
M.~Asberg, T.~Nolte, M.~Joki, J.~Hogbrink, and S.~Siwani.
\newblock Fast linux bootup using non-intrusive methods for predictable
  industrial embedded systems.
\newblock In \emph{Emerging Technologies \& Factory Automation (ETFA), 2013
  IEEE 18th Conference on}, pages 1--8. IEEE, 2013.

\bibitem[Bird(2004)]{bird04_methods}
T.~R. Bird.
\newblock Methods to improve bootup time in linux.
\newblock In \emph{Linux Symposium}, volume~1, pages 79--88, 2004.

\bibitem[Bovet and Cesati(2005)]{bovet2005understanding}
D.~P. Bovet and M.~Cesati.
\newblock \emph{Understanding the Linux kernel}.
\newblock " O'Reilly Media, Inc.", 2005.

\bibitem[Edler et~al.(1988)Edler, Lipkis, and Schonberg]{edler88_process}
J.~Edler, J.~Lipkis, and E.~Schonberg.
\newblock \emph{Process management for highly parallel UNIX systems}.
\newblock Citeseer, 1988.

\bibitem[Gooch(2002)]{gooch02_advanced}
R.~Gooch.
\newblock Advanced boot scripts.
\newblock In \emph{Ottawa Linux Symposium}, page 176, 2002.

\bibitem[Jo et~al.(2009)Jo, Kim, Roh, and Lee]{jo09_improving}
H.~Jo, H.~Kim, H.-G. Roh, and J.~Lee.
\newblock Improving the startup time of digital tv.
\newblock \emph{Consumer Electronics, IEEE Transactions on}, 55\penalty0
  (2):\penalty0 721--727, 2009.

\bibitem[Joo et~al.(2006)Joo, Choi, Park, Chung, Chung, and
  Chang]{joo06_demand}
Y.~Joo, Y.~Choi, C.~Park, S.~W. Chung, E.~Chung, and N.~Chang.
\newblock Demand paging for onenand™ flash execute-in-place.
\newblock In \emph{Proceedings of the 4th international conference on
  Hardware/software codesign and system synthesis}, pages 229--234. ACM, 2006.

\bibitem[Kaminaga(2006)]{kaminaga2006improving}
H.~Kaminaga.
\newblock Improving linux startup time using software resume (and other
  techniques).
\newblock In \emph{Linux Symposium}, page~17, 2006.

\bibitem[Kozuch and Wolfe(1994)]{kozuch94_compression_of_embedded}
M.~Kozuch and A.~Wolfe.
\newblock Compression of embedded system programs.
\newblock In \emph{Computer Design: VLSI in Computers and Processors, 1994.
  ICCD '94. Proceedings., IEEE International Conference on}, pages 270--277,
  Oct 1994.
\newblock \doi{10.1109/ICCD.1994.331903}.

\bibitem[Krishnakumar(2005)]{krishnakumar2005kernel}
R.~Krishnakumar.
\newblock Kernel korner: kprobes-a kernel debugger.
\newblock \emph{Linux Journal}, 2005\penalty0 (133):\penalty0 11, 2005.

\bibitem[McKenney(2007)]{paul07_rcu_fundamental}
P.~E. McKenney.
\newblock What is rcu, fundamentally?
\newblock \emph{LWN}, Nov. 2007.
\newblock \url{https://lwn.net/Articles/262464/}.

\bibitem[Mewburn(2001)]{mewburn01_design}
L.~Mewburn.
\newblock The design and implementation of the netbsd rc. d system.
\newblock In \emph{USENIX Annual Technical Conference, FREENIX Track}, pages
  69--79, 2001.

\bibitem[Miller(1968)]{miller1968response}
R.~B. Miller.
\newblock Response time in man-computer conversational transactions.
\newblock In \emph{Proceedings of the December 9-11, 1968, fall joint computer
  conference, part I}, pages 267--277. ACM, 1968.

\bibitem[Mochel(2005)]{mochel05_sysfs}
P.~Mochel.
\newblock The sysfs filesystem.
\newblock In \emph{Linux Symposium}, page 313, 2005.

\bibitem[Nakamura et~al.(2009)Nakamura, Igaki, Kimura, and
  Matsumoto]{Nakamura09_APSCC_service_candidates}
M.~Nakamura, H.~Igaki, T.~Kimura, and K.-i. Matsumoto.
\newblock Extracting service candidates from procedural programs based on
  process dependency analysis.
\newblock In \emph{Services Computing Conference, 2009. APSCC 2009. IEEE
  Asia-Pacific}, pages 484--491, Dec 2009.
\newblock \doi{10.1109/APSCC.2009.5394081}.

\bibitem[Oh et~al.(2006)Oh, Park, Lim, Lim, Oh, Kim, Shin, Song, Ryoo, Lim,
  Park, Kim, Kim, Yu, Yeung, Jeong, Kong, Kang, Koh, Jeong, Jeong, and
  Kim]{nvram_oh06_512mb_pram}
J.~Oh, J.~Park, Y.~Lim, H.~Lim, Y.~Oh, J.~Kim, J.~Shin, Y.~Song, K.~Ryoo,
  D.~Lim, S.~Park, J.~Kim, J.~Kim, J.~Yu, F.~Yeung, C.~Jeong, J.~Kong, D.~Kang,
  G.~Koh, G.~Jeong, H.~Jeong, and K.~Kim.
\newblock Full integration of highly manufacturable 512mb pram based on 90nm
  technology.
\newblock In \emph{Electron Devices Meeting, 2006. IEDM '06. International},
  pages 1--4, Dec 2006.
\newblock \doi{10.1109/IEDM.2006.346905}.

\bibitem[Owaki et~al.(1968)Owaki, Nakayama, Miyauchi, Tanaka, and
  Hori]{owaki68_new_crt_conf}
K.~Owaki, N.~Nakayama, E.~Miyauchi, M.~Tanaka, and K.~Hori.
\newblock A new type of cathode-ray tube with a crossed-field gun.
\newblock In \emph{Electron Devices Meeting, 1968 International}, volume~14,
  pages 40--40, 1968.
\newblock \doi{10.1109/IEDM.1968.187970}.

\bibitem[Owaki et~al.(1969)Owaki, Nakayama, Miyauchi, Tanaka, Hori, and
  Omori]{oawaki69_new_crt_journal}
K.~Owaki, N.~Nakayama, E.~Miyauchi, M.~Tanaka, K.~Hori, and K.~Omori.
\newblock A new type of cathode-ray tube with a crossed-field gun.
\newblock \emph{Electron Devices, IEEE Transactions on}, 16\penalty0
  (12):\penalty0 995--1001, Dec 1969.
\newblock ISSN 0018-9383.
\newblock \doi{10.1109/T-ED.1969.16899}.

\bibitem[Paul E.~McKenney(1998)]{paul98_rcu_concurrency}
J.~D.~S. Paul E.~McKenney.
\newblock Read-copy update: Using execution history to solve concurrency
  problems.
\newblock In \emph{Parallel and Distributed Computing and Systems}, pages
  509--518, Oct 1998.

\bibitem[Piggin(2008)]{ticket_spinlocks}
N.~Piggin.
\newblock Ticket spinlocks.
\newblock \emph{LWN}, Feb. 2008.
\newblock \url{https://lwn.net/Articles/267968/}.

\bibitem[Royon and Fr{\'{e}}not(2007)]{Royon07_CoRR_init-survey}
Y.~Royon and S.~Fr{\'{e}}not.
\newblock A survey of unix init schemes.
\newblock \emph{CoRR}, abs/0706.2748, 2007.
\newblock URL \url{http://arxiv.org/abs/0706.2748}.

\bibitem[Stallman(2014)]{fsf_opposing_drm}
R.~Stallman.
\newblock Opposing digital rights mismanagement.
\newblock \emph{FSF}, Nov. 2014.
\newblock \url{http://www.gnu.org/philosophy/opposing-drm.en.html}.

\bibitem[Tehrani et~al.(1999)Tehrani, Slaughter, Chen, Durlam, Shi, and
  DeHerren]{nvram_tehrani99_mram}
S.~Tehrani, J.~Slaughter, E.~Chen, M.~Durlam, J.~Shi, and M.~DeHerren.
\newblock Progress and outlook for mram technology.
\newblock \emph{Magnetics, IEEE Transactions on}, 35\penalty0 (5):\penalty0
  2814--2819, Sep 1999.
\newblock ISSN 0018-9464.
\newblock \doi{10.1109/20.800991}.

\bibitem[Whitaker()]{ken12_flash}
K.~Whitaker.
\newblock A comparative study of flash storage technology for embedded devices.

\bibitem[Zhuang et~al.(2002)Zhuang, Pan, Ulrich, Lee, Stecker, Burmaster,
  Evans, Hsu, Tajiri, Shimaoka, Inoue, Naka, Awaya, Sakiyama, Wang, Liu, Wu,
  and Ignatiev]{nvram_zhuang02_rram}
W.~Zhuang, W.~Pan, B.~Ulrich, J.~Lee, L.~Stecker, A.~Burmaster, D.~Evans,
  S.~Hsu, M.~Tajiri, A.~Shimaoka, K.~Inoue, T.~Naka, N.~Awaya, A.~Sakiyama,
  Y.~Wang, S.~Liu, N.~Wu, and A.~Ignatiev.
\newblock Novel colossal magnetoresistive thin film nonvolatile resistance
  random access memory (rram).
\newblock In \emph{Electron Devices Meeting, 2002. IEDM '02. International},
  pages 193--196, Dec 2002.
\newblock \doi{10.1109/IEDM.2002.1175811}.

\end{thebibliography}

==> old/subsection-archive/0510_OBSOLETE_design-core-engine.tex <==
%%%%%%%%%% OBSOLETE DO NOT USE %%%%%%%%%%%%%%
\error!!!

\subsection{Core Engine}\label{SS_core_engine}

The role of Core Engine located in kernel space is to enable
\emph{RCU Booster} and \emph{On-demand Modularizer} and start
the first user process (\textit{systemd} in our case) earlier
with additional mechanisms described below.

Memory Init
RCU Booster
On-demand Modulation



%\textbf{Kernel-level core engine to handle complicated software.} There are increasing the execution time of 
%the kernel initialization because of continuous complexity increase of the kernel and size increase of that. 
%We designed and implemented new kernel level core engine to improve drastically the increased execution time of 
%the kernel such as Figure~\ref{fig:operation-flow-of-core-engine}. 
%The major role of the core engine is to switch the init kernel thread to the user-space 
%as soon as enabling \emph{boosted RCU} facility and \emph{On-demand modulation} facility 
%after finishing a memory initialization based on the actual used memory size for faster initialization of the software stack. 
%The proposed core engine consists of major four functions; memory initialization of needed memory size 
%for software platform, boosting facility of RCU synchronization operation, on-demand kernel modulation 
%for built-in kernel features, and selective mounting mode between system and user partition. 

\begin{figure}
\centering
\includegraphics[width=0.4 \columnwidth,height=1.0in]{img/operation-flow-of-core-engine.png}
\caption{Operation flow of core engine}
\label{fig:operation-flow-of-core-engine}
\end{figure}

%Rethinking the Journaling costs of filesystem. Table 1 shows the operation flow 
%between normal boot and quick boot in the core engine. The rootfs mounting task of 
%the core engine operates with three types of mounting modes based on up-to-date 
%EXT4 filesystem~\cite{cao2007ext4} as follows:
%\begin{itemize} 
%\item 
%Journal mode:~\cite{prabhakaran05_journaling_evolution} 
%\emph{Metadata and data blocks} are committed 
%into the journal prior to being written into the main file system.  
%Enabling this mode will disable the delayed allocation and \emph{O\_DIRECT} [5] support.
%\item 
%Ordered mode:~\emph{Metadata} has been committed to the journal area 
%after its data blocks are forced directly out to the main file system. 
%In the embedded devices, 
%most of the software platform  operates the type of mounting mode by default. 
%\item  
%Writeback mode:~\emph{Data ordering} is not preserved, 
%data may be written into the main file system 
%after its metadata has been committed to the journal.
%\end{itemize} 
% If boot-up mode is a normal boot, the core engine attempts a mounting task with ordered mode 
% to commit all data of the file system. If the boot-up mode is a quick boot, 
% the core engine does attempt to perform a mounting task with \emph{writeback mode} 
% without any journaling of the file system among the three data modes 
% to reduce a mounting time of the file system. 
% However, the \emph{writeback mode} does not guarantee the complete recovery in case of 
% the unexpected operation such as a system crash or a power failure.  
% The initialization task of read-only system does not make data inconsistency according 
% to the \emph{writeback mode} even though power failure happens at boot time. 
% Therefore, we can safely maintain the \emph{wirteback mode} of read-only system partition.  
% After booting procedure of the system completes, we changed the mounting mode of 
% the writable user partition from \emph{writeback mode} to \emph{ordered mode} (e.g. \texttt{–o remount, data=writeback}) 
% to guarantee the file consistency of user partition that file write operation was happened frequently. 
% Figure~ref{fig:performance-complare-mount-mode} shows a performance comparison 
% when we run the mounting file system to 
% the physical storage with two different mounting modes.   

\begin{figure}
\centering
\includegraphics[width=0.5 \columnwidth,height=1.8in]{img/performance-complare-mount-mode.png}
\caption{Performance comparison by data mode of file system to mount storage}
\label{fig:performance-complare-mount-mode}
\end{figure}

\textbf{Increasing memory capacity causes slow memory initialization.} Also, quick boot initializes 
the physical memory size that is actually used at boot time for accelerating the startup time of the smart device. 
Figure~\ref{fig:mem-init-speed} shows the memory initialization cost of memory initialization 
when we set up the actual needed memory size (e.g., 512M, 1G, 1.5G, 2G) to observe the initial screen 
of the software stack. The memory initialization function marks the free areas [7] in the memory map [8] 
and tells us the amount of free memory. The architecture setup function is responsible
for architecture-specific initialization procedures. The architecture setup function includes 
setting up the machine vector and determining the locations and sizes of available memory. \cite{lim13_virtual}
The architecture setup function also initializes a basic memory allocator to use during the boot process, 
and for most processors, calls paging initialization function to enable the host's \emph{memory management unit (MMU)}. 
The rest initialization function frees the memory used by initialization functions, 
and then launches init function 
as a kernel thread to finish the kernel's boot process.

\begin{figure}
\centering
\includegraphics[width=0.6 \columnwidth,height=1.4in]{img/mem-init-speed.png}
\caption{Comparison of memory initialization time to acquire free pages at boot-up with different memory size}
\label{fig:mem-init-speed}
\end{figure}

The others refer to all of the kernel functions except for architecture setup, memory initialization, 
and rest initialization function during kernel initialization.\\
\textbf{On-demand modulation for built-in kernel subsystems.} Next, the kernel thread always executes 
\emph{initcall()} the kernel function to run a one-time initialization when the device drivers are loaded into the memory. 
An \emph{initcall ( )} is the initialization function for a module which is statically linked into the Linux kernel. 
We adopted the kernel module method without the kernel built-in method because the running of 
the \emph{initcall} mechanism consumes a large amount of time at boot-up. 
Finally, the core engine runs the mounting work of the file system and switches the init kernel thread 
to user land (e.g., \texttt{/sbin/init}) by executing the \emph{do\_execve()} kernel function.\\

Figure~\ref{fig:ondemand-builtin-modulation} show how on-demand modulation is operated at runtime. 
An \emph{initcall} is the initialization function for a module which is statically linked into the Linux kernel. 
Running of initcalls can consume a large amount of time during boot-up.
However, some modules do not need to be initialized so early, in order for the embedded device 
to become usable for its primary purpose. These initcalls can be run later, after first boot 
and possibly first use has completed. The \emph{/proc/deferred\_initcalls} will cause the kernel 
to run all deferred initcalls. Also the \emph{.init} section memory is freed by kernel. 
The contents of \emph{/proc/deferred\_initcalls} will return 0 if deferred initcalls were not yet run 
and 1 otherwise on subsequent reads. Then, kernel registers the capability of the kernel feature 
to manage data structure of built-in kernel features. 
When the built-in kernel features are requested via procfs \cite{Mouw01_procfs} interface 
by device-centric user applications. 
Finally, \emph{do\_function()} executes to proceed the service request of the user applications 
as a kernel itself without the external kernel module.\\

For example, many digital devices have \emph{Universal Serial Bus(USB)} buses, which need to be initialized in order 
for the camera to be used as a mass storage device to download pictures to a laptop computer. 
However, the USB buses do not need to be initialized for the primary use of the digital devices, 
which is to take pictures. In order to be able to take a picture as soon as possible after booting, 
initialization of the USB system in the kernel can be deferred until 
after completing the primary boot sequence for the digital devices.


\begin{figure}
\centering
\includegraphics[width=0.5 \columnwidth,height=1.7in]{img/ondemand-builtin-modulation.png}
\caption{On-demand execution structure of built-in kernel features}
\label{fig:ondemand-builtin-modulation}
\end{figure}

\textbf{Improving service scheduling with HZ.} Figure~\ref{fig:rcu-bottleneck}
shows pseudo code 
on the locking mechanism of container-based init scheme that aggregates processes
with OS-level lightweight container are called 
\texttt{}{Control-group}.[24] In this flow, the synchronized RCU function~\cite{paul07_rcu_fundamental} 
such as \emph{synchronize\_rcu( )} has to wait until a \emph{grace period}(such as context switch, idle loop, or user code) has elapsed.~\cite{paul01_rcu},
~\cite{har07_lockless_sync},~\cite{mckenney2011parallel} 
A \emph{grace period} is a quiescent state that each thread resides at least once. In other words, 
after all currently executing RCU read-side critical sections have completed. 
We can process the services quickly 
by accelerating the RCU locking mechanism (e.g. synchronized RCU function) at boot time. 
Operating system runs process scheduling according to the scheduler tick. 
If we try to increase the number of HZ to get the high precision, we can get the fine-grained scheduling infrastructure.

\begin{figure}
\centering
\includegraphics[width=0.5 \columnwidth,height=1.6in]{img/rcu-bottleneck.png}
\caption{Performance bottleneck while creating tasks by OS-level container based init; (left) is function flow of init 
to attach new task into a container, (right)  refers to the location of \emph{synchronize\_rcu} function of RCU mechanism~\cite{paul15_locking_performance} that is analyzed as a performance bottleneck by \texttt{}{Kprobe/Ftrace}~\cite{kprobe},~\cite{steven09_ftrace}.}
\label{fig:rcu-bottleneck}
\end{figure}


Figure~\ref{fig:hz-time-gap} shows that the tuning of the number of the HZ will improve the execution time of 
services at boot time. However, the number of HZ is dependent on the CPU architecture. 
As a trade-off, when timer interrupt handler is called more frequently because of the high number of HZ, 
CPU operation and power consumption will go up. Above all, most of the kernel facilities operate 
based on the number of HZ. So, the changing of the HZ number is not practical in real environment. 


\begin{figure}
\centering
\includegraphics[width=0.5 \columnwidth,height=1.4in]{img/hz-time-gap.png}
\caption{Time gap between former service and latter service with HZ tuning. The default Hz of 
ARM architecture is 100 Hz.}
\label{fig:hz-time-gap}
\end{figure}

\textbf{Restructure Synchronization facility.} \texttt{SPINLOCK} is helpful when process should not be put to sleep 
by interrupt service routines. We design to use the \texttt{SPINLOCK} mechanism when lock will be granted in reasonably 
short time after CPU-intensive startup time.
~\cite{paul98_rcu_concurrency},~\cite{cao03_rcu_for_ipc}
On the other hand, \texttt{MUTEX} is helpful to support fast execution of services when putting process is not 
harmful such as user space services of digital television at boot time. 
In this case, we designed the lightweight locking operation with \texttt{MUTEX} mechanism 
when there will be considerable time before process gets the lock.
In Figure~\ref{fig:rcu-naive-vs-boosted}, the boosted synchronization facility waits 
for an RCU-preempt grace period, but processes it quickly. The key approach is 
to invoke schedulable boosted synchronization function to push all the tasks to data structure of 
the blocked task lists and wait for this list to drain. It consumes significant time on all CPUs such as 
Figure~\ref{fig:cpu-usage-eval-naive-vs-boostedrcu} and is not appropriate to mission critical real-time systems. 
Therefore, we do not recommend for any sort of common-case environment.
If we must use to accelerate the synchronization operation with RCU facility in a loop, 
we may restructure the locking operation with \texttt{sysfs} ABI interface \cite{mochel05_sysfs} to batch RCU updates.

\begin{figure}
\centering
\includegraphics[width=0.7 \columnwidth,height=2.6in]{img/rcu-naive-vs-boosted.png}
\caption{Naive RCU mechanism VS boosted RCU mechanism}
\label{fig:rcu-naive-vs-boosted}
\end{figure}

\textbf{Boosted RCU mechanism.} The \emph{boosted synchronization} facility of the locking operations 
has the same semantics as the non-boosted locking structure, but boosting is both expensive 
and not friendly to workloads of real-time tasks.  Use of the \emph{boosted RCU} mechanism 
should be restricted to rare configuration-change operations that would not normally be undertaken 
while a real-time workload is running. In particular, in case of invoking one of the boosted synchronization facilities 
repeatedly in a loop, we can dynamically restructure the locking operation with \texttt{sysfs} based \emph{dynamic booster} 
in order that RCU mechanism batches the updates, allowing a single non-boosted primitive to cover the entire batch. 
This will very likely be faster than the loop containing the boosted synchronization facility, 
and will be much easier on the rest of the system, especially to real-time system running 
on the rest of the system. In addition, the boosted primitives are illegal 
to call the boosted procedure from a \emph{CPU hot-plug} infrastructure
and to call the boosted procedure 
while operating system is holding any lock that is acquired by a \emph{CPU hot-plug} infrastructure.  
Note that nonobservance of this restriction results in deadlock of the system.

\textrm{Experiment of boosted synchronization facility.} After the initialization procedure of the kernel, 
we compared the CPU utilization between \emph{naïve RCU} and \emph{boosted RCU} mechanism for booting time of the device. 
We figured out that CPU utilization is increased on 
average 15\%; from 70\% to 85\% such as Figure~\ref{fig:cpu-usage-eval-naive-vs-boostedrcu}. 
From our analysis, the major reason on the increase of the CPU utilization results 
from the \emph{waiting time (idle time)} of the processes. 

\begin{figure}
\centering
\includegraphics[width=0.5 \columnwidth,height=2.7in]{img/cpu-usage-eval-naive-vs-boostedrcu}
\caption{CPU Usage between Naive RCU and Boosted RCU}
\label{fig:cpu-usage-eval-naive-vs-boostedrcu}
\end{figure}

When we applied for our \emph{boosted RCU} mechanism into \emph{synchronize\_rcu( )} kernel synchronization function 
in \texttt{Linux kernel 3.10}, we could verify the reduction effect on waiting time of the processes such as Figure~\ref{fig:sync-cost-eval-naive-vs-boostedrcu}. 
We profiled the self-execution time of the synchronize\_rcu() function 
with \texttt{kernel Function TRACEer(FTRACE)}~\cite{steven09_ftrace}. From our analysis, 
Figure~\ref{fig:sync-cost-eval-naive-vs-boostedrcu} shows that our proposed boosted synchronization approach 
drastically improved the cost of synchronization at boot time from 23.7 msecs to 3.1 msecs on average 
against the existing naive synchronization facility. When the number of the services during the booting procedure, 
is 136 services, it means that we can reduce the execution time of 
the services 2801.6 msecs; 136 services * (23.7 msecs - 3.1 msecs). 
We could show that high synchronization time of processes was happened normally in the some ranges.
The locking processes of critical section was not preempted from the busy waiting processes 
according to the priority-based task scheduling because scheduling priority of the locking processes were higher than
the busy waiting processes.

\begin{figure}
\centering
\includegraphics[width=0.7 \columnwidth,height=1.6in]{img/sync-cost-eval-naive-vs-boostedrcu}
\caption{Experimental result of synchronization cost between naive RCU and boosted RCU}
\label{fig:sync-cost-eval-naive-vs-boostedrcu}
\end{figure}

==> old/subsection-archive/0520_OBSOLETE_design-bootup-engine.tex <==
\subsection{Boot-up Engine}\label{SS_bootup_engine}

%As described previously, Boot-up Engine defers non booting critical \textit{systemd} tasks
%with Deferred Executor and manages two features, RCU Booster and On-demand Modularizer, implemented by
%Core Engine. Deferred Executor defers the following \textit{systemd} tasks.

%\textit{Logging service}, which is started at the earlier phase of \textit{systemd} booting, is
%deferred until the system recognizes a completion of booting.
%Setup procedures of kernel modules, hostname, machine ID, loopback device, and
%directories with test and debug purposes are also deferred until the booting completion.
%Another big

%\textbf{Postpone unnecessary functions at boot time.} The boot-up engine sets up the initial system environment 
%of the root file system after finishing the logging mechanism, mounting file system, and loading configuration files. 
%Figure \ref{fig:operation-flow-of-bootup-engine} shows the difference in operation structure between the normal boot 
%and quick boot during the execution duration of the boot-up engine. 
%The disadvantage of the existing system is that too many resources, such as CPU and I/O, 
%are used instead of supplying helpful logging messages during booting time. We do not needed 
%enabling the logging messages after debugging task in the development period because 3rd party applications of 
%the users are executed after completing the booting procedure of the system.

\begin{figure}
\centering
\includegraphics[width=0.4 \columnwidth,height=1.3in]{img/operation-flow-of-bootup-engine.png}
\caption{Operation flow of boot-up engine}
\label{fig:operation-flow-of-bootup-engine}
\end{figure}

Therefore, a quick boot enables the logging operation after finishing the booting procedure 
to accelerate the startup time of the smart device.\\
\textbf{Accelerate service execution with Dynamic booster.} The boosted RCU locking mechanism 
of the core engine has the structure of pre-emptible locking facility. 
Therefore, it can control fine-grained process scheduling. On the other hand, this operation consumes 
more CPU resource compared to the existing locking mechanism. 
From our experiments, we verified that boosted RCU locking mechanism used CPU resource 
more than CPU usage ratio of 10~15\%. The boosted RCU locking facility is helpful to 
improve the boot time of the devices. Then, this mechanism can be applied for CPU-aware embedded devices 
by user-space controller. We implemented the run-time locking facility of user-space 
by connecting the kernel-level synchronization equipment and user-space controller via \texttt{sysfs} \cite{mochel05_sysfs}. 


\begin{figure}
\centering
\includegraphics[width=0.7 \columnwidth,height=1.9in]{img/effect-of-dynamic-booster.png}
\caption{Effects of dynamic booster at boot engine}
\label{fig:effect-of-dynamic-booster}
\end{figure}

Figure \ref{fig:effect-of-dynamic-booster} shows the effect of the \emph{dynamic booster}, 
which controls the locking mechanism dynamically in the run-time. 
We could verify that the \emph{dynamic booster} 
can drastically reduce the time gap between start time of the former service
and that of the latter service 
when we disabled the boosted locking operation using \texttt{sysfs}. \cite{mochel05_sysfs}

%\begin{lstlisting}
%[service-extension-framework.service]  
%[Unit]
%Description=Service extension framework broker daemon
%[Service]
%Type=oneshot
%ExecStart=/bin/sh -c '/bin/echo 0 > /sys/kernel/boosted_sync'
%ExecStart=/usr/bin/broker-daemon
%[Install]
%WantedBy=multi-user.target
%\end{lstlisting}

==> old/subsection-archive/0530_OBSOLETE_design-service-engine.tex <==
%\subsection{Service Engine}\label{SS_service_engine}
%\textbf{Find boot-time critical services.} Table 3 shows the operation structure of the service engine, 
%illustrating how the service engine handles the normal boot and quick boot. 
%The service engine makes an independent quick boot group to overcome the dependencies 
%among the applications when the init process loads the configuration files such as the operation flow 
%of service engine in Figure~\ref{fig:operation-flow-of-service-engine} (right picture). 
%The engine removes the complexity of the dependency that interrupts to speed up startup time 
%by separating completely the dependency relationship from another group at the booting time. 
%Moreover, the engine executes alphabet sorting to decide execution sequence among the services 
%in Quickboot group without any dependency statements to improve the calculation cost of dependency sequence. \\
%\begin{figure}
%\centering
%\includegraphics[width=0.4 \columnwidth,height=1.4in]{img/operation-flow-of-service-engine.png}
%\caption{Operation flow of service engine}
%\label{fig:operation-flow-of-service-engine}
%\end{figure}
%Service engine can define the boot-time critical services by drawing the graph on 
%call relationship between the services, which have dependency relationship with launcher software. 


% Isolation 이야기는 background에서 뺍니다. (going to design)
%In Figure~\ref{fig:dependency-by-new-service} , the start time of \emph{service a} is
%after start up of group a, which manages new \emph{service c}. the execution delay of
%the service a postpones the start time of the application launcher which shows
%users initial screen of the devices, by deferring the execution of the service b in \emph{group c}. 
%In this case, we can run an independent execution by completely isolating
%one process from the other processes in order to get the constant start
%time of the services.
%As a result, we can drastically minimize the waiting time of the users that
%must continue until the boot-up procedure terminates.\\
%\textbf{Isolate boot-time critical services.} The execution sequence of the services is decided by the unit of the service file
%without the that of the group name.
%Figure~\ref{fig:dependency-by-new-service} (c) shows how creation of the new \emph{service c} 
%affects the changes of the service's call relationship.
%Figure~\ref{fig:dependency-by-new-service}  (b) shows that creation of the new \emph{service c} 
%can change start time of the existing service.
% New \emph{service c} appended new dependency relationship to execute the tasks 
% before starting the creation of the existing \emph{service a}.
% In this case, execution sequence of the \emph{service a} in group b, can be delayed.
% The group is in charge of grouping the services, which have same execution characteristics.
% It supports the facility, which can start the services of the next group 
% when all services of same group are completed.
%However, even though the services of same characteristics is in one group together, 
%dependency-based service start method cannot guarantee that dependency relationship of new services 
%keep the original attribute of the group.
%As a result of that, the existing \emph{group b} can be divided into two groups logically.
%The creation and dependency addition of the new service can destroy constant start time 
%of the service a, which is completed within the existing \emph{group b}. \\
%To avoid the delay of the services, quickboot group completely isolates the service from 
%the attempt of the other services. Above all, the services of the quickboot group are executed 
%in order without any parsing procedure of the services' execution sequence 
%by deciding the start time of the service using number prefix rule such as \emph{“001-service-name”}.\\

%\subsection{Service analyzer and Service pre-parser}

%\textbf{Monitor conflicts of dependency among the services.} If new service file is appended by service developer, 
%dependency relationship of another service is added due to the new service. 
%When dependency structures of the service files are complicated or service developer try 
%to define unnecessary dependency relationship of a service, call sequence of the services 
%can be changed such as Figure \ref{fig:dependency-by-new-service}. 
%At this time, start time of the correct service files will not be guaranteed in case that the developers 
%define incorrect call relationship of the services. 
%To avoid this case, we implemented \textit{service dependency analyzer}, 
%which report the incorrect dependency structure of the services by checking the loop range of the services 
%because of the duplex call structure 
%using the existing open source call-graph generators; \textbf{Codeviz}~\cite{codeviz} and \textbf{Graphviz}.~\cite{graphviz} 
%Figure \ref{fig:infinite-loop-finding} shows that infinite loop can be founded by duplex call structure, 
%which calls each other. Red arrows refer to the conflict status of the services due to the infinite loop. \\
%\begin{figure}
%\centering
%\includegraphics[width=1.0 \columnwidth,height=1.0in]{img/construction.png}
%\caption{Caller/callee relationship between graphical.target and others; Black = Requires, 
%Dark blue = Requisite , Dark grey = Wants, Red = Conflicts, Green = After}
%\label{fig:infinite-loop-finding}
%\end{figure}
%\textbf{In memory service loader.} All services have configuration files, which defined self-dependency 
%against another service. For example, when init process have to execute 200 services at boot time, 
%the other services may start their tasks after finishing the booting procedures for faster booting of the devices. 
%Therefore, we introduced \emph{"deferred execution"} technique, which execute after completing the execution of 
%the launcher software. However, loading and parsing cost on configuration files of 200 services is dependent 
%on the complexity of the configuration files. We implemented \emph{"in-memory service loader"} to remove these costs 
%at boot time. It is in charge of the integrating the 200 service's configuration files to decoded one file 
%before releasing commercial devices. As a result, we can remove the execution cost of the 200 call operations 
%of open system call for 200 services. Also, parsing cost of 200 services' configuration files were not happened 
%at boot time of the devices. We fortunately executed pre-parsing operation just once because 200 services 
%were developed by the manufacturers without the third-party application developers.

==> old/subsection-archive/disable_030_relatedwork.tex <==
%% OBSOLETE. MERGED INTO BACKGROUND


\emph{\textbf{Suspend and Restore:}} We have been applying two suspend-and-restore 
based techniques for faster booting in consumer electronics: hibernation-based
snapshot booting~\cite{snapshot_boot} and suspend-to-RAM~\cite{suspend-to-RAM}.
For traditional consumer electronics where third party applications and
application stores are not considered, the hibernation technique has provided
very fast booting even for Linux-based embedded devices. For example, NX-300M
cameras with Linux-based Tizen OS (application stores excluded) have achieved
near 1 second of booting time~\cite{NX300M_Booting} with snapshot booting. Such
devices have limited variations in their initial states after a boot, which in
turn, allow to use preloaded ``factory'' snapshot images. If users may install
third party applications and services as smart phones and smart TVs allow,
preloaded snapshot images become useless and the device should create snapshot
images in run-time, which is hard to implement with enough reliability for
manufacturers. Users may plug off power cords or pull out batteries at any time
and creating a snapshot image takes a lot of time and users cannot use the
device in the middle of the process. Enforcing users to wait for tens of
seconds with no responses for every application installation or shutdown is
even worse than tens of seconds for booting. Besides, with large size of RAM,
snapshot booting may take a lot of time. For example, the UFS 2.0 storage
of Galaxy S6 with Exynos 7420, which is one of the most advanced storages for embedded systems,
may read sequentially at about 300~MiB/s~\cite{galaxy_s6_ufs_benchmark},
which translates to about 10 seconds to read contents of 3~GiB DRAM.\\


Suspend-to-RAM has been widely applied to consumer electronics: smart phones,
TVs (``instant on''~\cite{Samsung_Instant_On}), cameras (NX300M also uses this
if users turn on the camera not long after turning it off), and watches. One
critical requirement of Suspend-to-RAM is to supply power to the device while
the device is supposed to be turned off. For battery operated devices, this
might not a issue. For TVs, many users plug off TVs frequently, prohibiting
suspend-to-RAM and complains of slow booting and putting batteries to TVs
incurs significant additional manufacturing costs and requires TV developers to
optimize power consumption so that TV sets do not consume too much while
``suspended''. Thus, we cannot rely on suspend-to-RAM for TVs (and other
plugged-in consumer electronics) and we should make a cold boot--booting up the
device from a clean RAM and with conventional booting sequences--fast enough.\\


\emph{\textbf{Non-Volatile RAM (NVRAM) Based Approach:}} Tim
Bird~\cite{bird04_methods} has suggested to use execution-in-place
(XIP) with non-volatile RAM (NVRAM) to improve booting performance. The
introduction of NVRAM as fast as (or faster than) DRAM such as
MRAM~\cite{MRAM}, PRAM~\cite{PRAM}, and RRAM~\cite{RRAM} may shine lights on
this approach; however, high density high-performing NVRAM is still too
expensive for mass production~\cite{dontknowyet}. Affordable NVRAM provides
only tens of MiBs at this point; 32MiB STT-MRAM costs tens of US
dollars~\cite{sttmram_pricing}. Intel and Micron have announced their mass
production plan for 3D Cross Point memory, which is claimed to be slightly
slower than DRAM while it is non-volatile and high-density ~\cite{3DCROSSPOINT}.
As we do not have any affordable high-density and high-performing NVRAM
available at this point and we do not expect to have one soon enough, 
we do not rely on such technologies in this study.\\


\subsection{Compression}\label{SS_relatedwork_compression}
In the past, the storage I/O throughput of consumer electronics had been
the major bottleneck for faster booting.
The I/O throughput is especially critical if the system relies on
hibernation-based snapshot booting.

Note that compression does not help much because the flash I/O throughput overwhelms
the decompression throughput: 35~MiB/s, running all 8 cores of Exynos 7420 of Galaxy S6~\cite{galaxy_s6_geekbench}.\\


% Dependency 기반의 init scheme (systemd 전, abs 이후) 혹시 더 소개할 만한것 있나요?
\emph{\textbf{Dependency-based Init Scheme:}} Dependency-based init scheme
gurantees the correctness of booting sequences by invoking OS services
in the order based on the declared dependencies between services.
If such depedencies are not kept and a service is invoked (a process is started),
the service may not start correctly and the whole booting sequence might be
jeopardized. For example, if Apache2 web server starts before the file system
containing its configurations (usually /etc/) is mounted, it might fail to start.\\

Advanced Boot Script~\cite{gooch02_advanced}
has proposed a dependency-based init scheme supporting parallelism and dependency
declaration. Advanced Boot Script allows software package
developers to declare uni-directional dependencies (e.g., ``I need service A initialized before me'')
for services
and initializes services in parallel if they are in a same group and do not
break the declared dependencies. The limitations of Advanced Boot Script
for boot time optimization are as follows. 1) It is based on run-levels,
which are groups subscribed by each program to be invoked at boot-time and 
run-levels are in a total order.
Programs in different run-levels cannot be invoked in parallel.
2) It does not allow system developers
(or administrators in server systems) to prioritize specific programs for faster
booting.
Note that \cite{gooch02_advanced} has focused to guarantee the correctness of booting sequence 
defined by dependency declarations and does not address 
the parallel execution between different run-levels or allow developers express
priorities between services.\\


% 중간에 Systemd 이야기 하고 전반적인 dependency 문제로 갑니다.
More advanced dependency-based init scheme, systemd~\cite{systemd_official_freedesktop}
has been widely accepted as the standard init scheme for Tizen and other various
major Linux distributions recently~\cite{systemd_wiki_adoption}:
Arch Linux, CoreOS, Debian, Fedora, Megeia, openSUSE, Red Hat Enterprise Linux,
Slackware, SUSE Linux Enterprise, and Ubuntu.
Dependencies, start-up priorities and conditions, resource management policies,
monitoring and recovery systems, and other related mechanisms for each service are
declared by the service in its own \emph{unit file},
which is parsed and served at boot time.\\


The advantages of systemd include
the removal of run-levels allowing more parallelism between start-ups of services
and the capabilities for more complex requirement expressions
for services. For example, a service may declare ``I am needed by service A'',
``I need to be started before service B'', or ``I need to be started if /tmp/foo is created.''
Systemd also provides mechanisms to monitor and manage the services in run time and to
provide resource management services to user processes. It has a lot of potential to
tweak and fine-tune the system with various tools for system and service developers.\\



Disadvantages of systemd incur mainly due to the complexity of systemd itself.
Allowing more tools and expressions for developers usually results in more chances
to abuse. We have witnessed many cases where service developers try to get higher
priorities and more resources than others to improve their services negatively impacting
the overall performance; i.e., the booting time.
They also often add unnessary dependencies in order to ensure the correctness of
their services only resulting in unnessarily invoking processes excessively
or even creating circular dependencies. With hundreds of processes running at
% Tizen TV 실제 제품에서의 unit file 개수하고 booting직후 process 갯수 구할 수 있을까요?
the initial state, system developers cannot have enough knowledges for such processes.
Thus, system developers cannot to cope with such issues
effectively especially when service developers change specifications day by day
until the products are shipped. Sometimes, they change specifications even after
the products are shipped!\\


% Systemd 이야기도 붙여주세요. (우리가 여기에 based on 했다는 이야기도 하려고요)
% 이 논리로 reader에게 어필을 하면 어떨지요? 
% 기존의 coarse-grained parallelism 한계를 극복하기 위하여, 
% 최근에 systemd가 modern Linux distributions 의 default init scheme 으로써 채택되었다.
% Systemd 는 run-level 단위 뿐만 아니라 service 단위까지 fine-grained parallel execution 지원한다.
% 우리는 제안 아이디어가 실용적인 솔류션임을 입증하기위하여 가장 popular한 init process systemd에 기반하여 Quick boot framework을 구현 및 적용하였다.

% 간단하게 자기자랑하며 마치기.
Our work is also based on systemd as all of our TV products are now based on Tizen.
The work does not require much knowledge on the OS services for system developers
who are working on the overall booting mechanisms (Linux kernel and systemd), resolving
major disadvantages of dependency-based init schemes.
Our system (Samsung Smart TV 2015 models) is not based on mechanisms with critical
drawbacks for modern consumer electronics while suspend-to-RAM techniques can still
be applied.
%혹시 Instant-On + Tizen TV가 있으면 같이 쓰면 되겠습니다.



==> old/subsection-archive/references.tex <==
% sources

%% LET's MOVE ON TO .bib FILE

%%% DEPRECATED.

\begin{thebibliography}{}
\bibitem{systemd}
Systemd, Lennart Poettering, reference text
%\bibitem{init-survey} --> bib / royon07_corr
%Y. V. Royon and S. Frénot, “A Survey of Unix Init Schemes,” In Proceedings of  CoRR, Jun. 2007.
%%%(moved to .bib)bibitem{TBD}
%M. Nakamura, H. Igaki, T. Kimura, and K. Matsumoto, “Extracting service candidates from procedural programs based on process dependency analysis,” In Proceedings of IEEE Asia-Pacific Services Computing Conference (APSCC), 2009.
%%%(moved to .bib)bibitem{TBD}
%E. Mouw, “Linux kernel procfs guide,” Faculty of Information Technology and Systems, 2001.
%%%(moved to .bib)bibitem{TBD}
%P. Mochel, “The sysfs filesystem,” In Proceedings of Linux Symposium, 2005.
\bibitem{TBD}
L. Tovalds, “O\_DIRECT performance impact on 2.4.18,” Electronic message to the linux-kernel mailing list. Message-ID: fa.m6umeav. 15008gs@ ifi. uio. 2002
%%%(moved to .bib)bibitem{TBD}
%V. Prabhakaran, C. A. Andrea, and H. A. Remzi, “Analysis and Evolution of Journaling File Systems,” In Proceedings of USENIX Annual Technical Conference (ATC), 2005.
%%%(moved to .bib)bibitem{TBD}
%G. Lim, G. Min, and Y. I. Eom, “Virtual memory partitioning for enhancing application performance in consumer electronics,” IEEE Transactions on Consumer Electronics, issue 4, vol. 59, pp. 786-794, Nov. 2013
%%%(moved to .bib)bibitem{TBD}
%H. Jo, H. Kim, H. Roh, and J. Lee, “Improving the startup time of Digital TV,” IEEE Transactions on Consumer Electronics, Aug. 2009.
%%%(moved to .bib)bibitem{TBD}
%M. S. v. Bennewitz, “Chances for a tizen smartphone entry,” Linux Journal, 2013.
%%%(moved to .bib)bibitem{TBD}
%R. Gooch, “Advanced boot scripts,” In Proceedings of Linux Symposium. pp. 176-182, Jun. 2002.
%%%(moved to .bib)bibitem{TBD}
%M. Asbert, T. Nolte, M. Joki, J. Hogbrink, and S. Siwani, “Fast Linux boot-up using non-intrusive methods for predictable industrial embedded systems,” In Proceedings of Emerging Technologies \& Factory Automation (ETFA), Sep. 2013.
%%%(moved to .bib)bibitem{TBD}
%J. Edler, J. Lipkis, and E. Schanberg, “Process management for highly parallel UNIX systems,” Ultracomputer Research Laboratory, Courant institue of mathematical sciences, 1988.
%%%(moved to .bib)bibitem{TBD}
%T. R. Bird, “Methods to improve boot-up time in Linux,” In Proceedings of Linux Symposium. pp. 79-88, 2004.
%%%(moved to .bib)bibitem{TBD}
%Y. Joo, Y. Choi, C. Park, S. W. Chung, E. Chung, and N. Chang,. “Demand paging for OneNAND™ Flash eXecute-in-place,” In Proceedings of the 4th international conference on Hardware/software codesign and system synthesis. ACM, 2006.
%%%(moved to .bib)bibitem{TBD}
%Luke Mewburn. 2001. The Design and Implementation of the NetBSD rc.d System. In Proceedings of the FREENIX Track: 2001 USENIX Annual Technical Conference, Clem Cole (Ed.). USENIX Association, Berkeley, CA, USA, 69-79
%%%(moved to .bib)bibitem{TBD}
%Gooch, Richard. "Advanced Boot Scripts." In Ottawa Linux Symposium, p. 176. 2002.
%%%(moved to .bib)bibitem{TBD}
%Adams, Jonathan, David Bustos, Stephen Hahn, David Powell, and Liane Praza. "Solaris Service Management Facility: Modern System Startup and Administration." In LISA, pp. 225-236. 2005.
%%%(moved to .bib)bibitem{TBD}
%Lim, Geunsik, Jae-young Hwang, Kyungmin Park, and Sang-Bum Suh. "Enhancing init scheme for improving boot-up time in consumer electronics." In Mobile Computing and Ubiquitous Networking (ICMU), 2015 Eighth International Conference on, pp. 149-154. IEEE, 2015.
%%%(moved to .bib)bibitem{TBD}
%Shabtai, Asaf, Yuval Fledel, and Yuval Elovici. "Securing Android-Powered Consumer electronics Using SELinux." IEEE Security \& Privacy 8, no. 3 (2010): 36-44. 
\bibitem{TBD}
Lennart Pottering, “Systemd: Beyond Init,” Linus Con, Aug. 2011. 
\bibitem{TBD}
Sysadmin Magazine, Z. Jedrzejewski-Szmek, "Daemon Management Under Systemd," USENIX, Vol. 40, No. 3, Jun-201 
\bibitem{TBD}
Systemd: http://freedesktop.org/wiki/Software/systemd/
\bibitem{TBD}
Preseed: https://wiki.debian.org/DebianInstaller/Preseed
\bibitem{TBD}
Installing without systemd, https://wiki.debian.org/systemd\#Installing\_without\_systemd
\bibitem{TBD}
Init: http://en.wikipedia.org/wiki/Init
\bibitem{TBD}
Upstart: http://en.wikipedia.org/wiki/Upstart
\bibitem{TBD}
Whitaker, Ken. "A Comparative Study of Flash Storage Technology for Embedded Devices."
\bibitem{TBD}
Debian fork: http://debianfork.org/
\bibitem{TBD}
Tizen, Tizen Association: http://www.tizen.org
\bibitem{TBD}
Samsung Opensource, Samsung Electronics,  http://oepnsource.samsung.com
\bibitem{TBD}
OpenSource Code Distribution, LG Electronics, http://opensource.lge.com    
\bibitem{TBD}
Sony Open Source Code Distribution Service, Sony Electronics, https://products.sel.sony.com/opensource/ 
\bibitem{TBD}
What is RCU, Fundamentally?, Paul E. McKenney, IBM Linux Technology Center, https://lwn.net/Articles/262464/
\bibitem{TBD}
McKenney, Paul E. "RCU vs. locking performance on different CPUs." linux. conf. au, Adelaide, Australia. 2004.
\bibitem{TBD}
McKenney, Paul E., et al. "Read-copy update." AUUG Conference Proceedings. AUUG, Inc., 2001.
\bibitem{TBD}
McKenney, Paul E., and John D. Slingwine. "Read-copy update: Using execution history to solve concurrency problems." Parallel and Distributed Computing and Systems. 1998.
\bibitem{TBD}
Arcangeli, Andrea, et al. "Using Read-Copy-Update Techniques for System V IPC in the Linux 2.5 Kernel." USENIX Annual Technical Conference, FREENIX Track. 2003.
\bibitem{TBD}
Hart, Thomas E., et al. "Performance of memory reclamation for lockless synchronization." Journal of Parallel and Distributed Computing 67.12 (2007): 1270-1285.
\bibitem{TBD}
Codevi,: A CallGraph Visualiser, ww.csn.ul.ie/~mel/projects/codeviz/
\bibitem{TBD}
Graphviz, Open source graph (network) visualization project from AT\&T Research, www.graphviz.org
\bibitem{TBD}
Kprobe, An introduction to KProbes,   Linux Weekly News, https://lwn.net/Articles/132196/ 
\bibitem{TBD}
Debugging the kernel using Ftrace,  Linux Weekly News, https://lwn.net/Articles/365835// 
\bibitem{TBD}
Cathode ray tube: General description, http://www.newworldencyclopedia.org/entry/Cathode\_ray\_tube
\bibitem{TBD}
Owaki, K.; Nakayama, N.; Miyauchi, E.; Tanaka, M.; Hori, K., "A new type of cathode-ray tube with a crossed-field gun," in Electron Devices Meeting, 1968 International , vol.14, 1968.
\bibitem{TBD}
Owaki, K.; Nakayama, N.; Miyauchi, Eizo; Tanaka, M.; Hori, K.; Omori, K., "A new type of cathode-ray tube with a crossed-field gun,", IEEE Transactions on Electron Devices, vol.16, no.12, pp.995-1001, Dec 1969.
\bibitem{TBD}
Patent, "Instant warm-up heater cathode", US 3895249 A, https://www.google.com/patents/US3895249, 1975
\bibitem{TBD}
Patent, "Fast warm up picture tube cathode cap having high heat emissivity surface on the interior thereof", https://www.google.com/patents/US3958146, US 3958146 A, 1976
\bibitem{TBD}
Patent, Quick-heating cathode structure, US 4388551 A, https://www.google.com/patents/US4388551, 1980
\bibitem{TBD}
Samsung, LGE and Sony to Account for Nearly Half of All TV Display Panels Shipping in 2015 , DisplayResearch, Press Release, http://www.displaysearch.com/cps/rde/xchg/displaysearch/hs.xsl/pr\_manage.asp, 2015
\bibitem{TBD}
Cooke, Jim. "The inconvenient truths of NAND flash memory." Micron MEMCON 7 (2007).
\bibitem{TBD}
Articles, eMMC to UFS: How NAND Memory for Mobile Products Is Evolving, http://global.samsungtomorrow.com/emmc-to-ufs-how-nand-memory-for-mobile-products-is-evolving/, 2015
\bibitem{TBD}
Kozuch, Michael, and Andrew Wolfe. "Compression of embedded system programs." Computer Design: VLSI in Computers and Processors, 1994. ICCD'94. Proceedings., IEEE International Conference on. IEEE, 1994.
\end{thebibliography}
